Private and Robust Distributed Nonconvex Optimization via Polynomial Approximation

There has been work that exploits polynomial approximation to solve distributed nonconvex optimization problems involving univariate objectives. This idea facilitates arbitrarily precise global optimization without requiring local evaluations of gradients at every iteration. Nonetheless, there remains a gap between existing guarantees and practical requirements, e.g., privacy preservation and robustness to network imperfections. To fill this gap and keep the above strengths, we propose a Private and Robust Chebyshev-Proxy-based distributed Optimization Algorithm (PR-CPOA). Specifically, to ensure both the accuracy of solutions and the privacy of local objectives, we design a new privacy-preserving mechanism. This mechanism leverages the randomness in blockwise insertions of perturbed vector states and hence provides a stronger privacy guarantee in the scope of ($\alpha,\beta$)-data-privacy. Furthermore, to gain robustness against network imperfections, we use the push-sum consensus protocol as a backbone and discuss its specific enhancements. Thanks to the purely consensus-type iterations, we avoid the privacy-accuracy trade-off and the bother of selecting proper step sizes in different settings. We rigorously analyze the accuracy, privacy, and complexity of the proposed algorithm. We show that the advantages brought by introducing polynomial approximation are maintained when all the above requirements exist.

==> section/biography.tex <==
% !TEX root = ..\article.tex

\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.5in,clip,keepaspectratio]{photo/hzy2}}]{Zhiyu He}
%(S'20)
(Student Member, IEEE) received the B.E.\ degree and the M.S.\ degree in Control Science and Engineering from Shanghai Jiao Tong University, Shanghai, China, in 2019 and 2022, respectively. He is currently a Ph.D.\ student at the Automatic Control Laboratory at ETH Z{\"u}rich and the Max-Planck ETH Center for Learning Systems. His research interests lie in distributed optimization, learning, and control of network systems.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.5in,clip,keepaspectratio]{photo/jphe3}}]{Jianping He}
%(M'15-SM'19) 
(Senior Member, IEEE) received the Ph.D.~degree in control science and engineering from Zhejiang University, Hangzhou, China, in 2013.

From December 2013 to March 2017, he was a Research Fellow with the Department of Electrical and Computer Engineering, University of Victoria, Victoria, BC, Canada. He is currently an Associate Professor with the Department of Automation, Shanghai Jiao Tong University, Shanghai, China. His research interests mainly include distributed learning, control and optimization, and security
and privacy in network systems.

%Dr.~He serves as an Associate Editor for IEEE Trans.~Control of Network Systems, IEEE Open Journal of Vehicular Technology, and KSII Trans.~Internet and Information Systems. He was also a Guest Editor of IEEE TAC, International Journal of Robust and Nonlinear Control, etc. He was the winner of Outstanding Thesis Award, Chinese Association of Automation, 2015. He received the best paper award from IEEE WCSP'17, the best conference paper award from IEEE PESGM'17, and was a finalist for the best student paper award from IEEE ICCA'17, and the finalist for best conference paper award from IEEE VTC'20-FALL.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.5in,clip,keepaspectratio]{photo/cailianchen2}}]{Cailian Chen}
%(S'03-M'06) 
(Member, IEEE) received the B.Eng.\ and M.Eng.\ degrees in automatic control from Yanshan University, Qinhuangdao, China, in 2000 and 2002, respectively, and the Ph.D. degree in control and systems from the City University of Hong Kong, Hong Kong, in 2006.

She has been with the Department of Automation, Shanghai Jiao Tong University, Shanghai, China, since 2008. She is now a Distinguished Professor. She has authored three research monographs and more than 100 referred international journal papers. She is the inventor of more than 20 patents. Her research interests include industrial wireless networks, computational intelligence and situation awareness, and Internet of vehicles.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.5in,clip,keepaspectratio]{photo/xpguan3}}]{Xinping Guan}
%(SM'04-F'18) 
(Fellow, IEEE) received the B.S.~degree in Mathematics from Harbin Normal University, Harbin, China, in 1986, and the Ph.D.~degree in Control Science and Engineering from Harbin Institute of Technology, Harbin, China, in 1999.

He is currently a Chair Professor with Shanghai Jiao Tong University, Shanghai, China, where he is the Dean of the School of Electronic Information and Electrical Engineering, and the Director of the Key Laboratory of Systems Control and Information Processing, Ministry of Education of China. Before that, he was the Professor and Dean of Electrical Engineering, Yanshan University, Qinhuangdao, China. His current research interests include industrial cyber-physical systems, wireless networking and applications in smart factory, and underwater networks.

% As a Principal Investigator, he has finished/been working on many national key projects. He is the leader of the prestigious Innovative Research Team of the National Natural Science Foundation of China (NSFC). He has authored and/or coauthored five research monographs, more than 270 papers in IEEE Transactions and other peer-reviewed journals, and numerous conference papers. 

% Dr.~Guan is an Executive Committee Member of Chinese Automation Association Council and the Chinese Artificial Intelligence Association Council. He was the recipient of the First Prize of Natural Science Award from the Ministry of Education of China in both 2006 and 2016, and the Second Prize of the National Natural Science Award of China in both 2008 and 2018, and the IEEE Transactions on Fuzzy Systems Outstanding Paper Award in 2008. He is a National Outstanding Youth honored by NSF of China, Changjiang Scholar by the Ministry of Education of China and State-level Scholar of New Century Bai Qianwan Talent Program of China.
\end{IEEEbiography}

